Estimating Total Correlation with Mutual Information Estimators

Total correlation (TC) is a fundamental concept in information theory that measures statistical dependency among multiple random variables. Recently, TC has shown noticeable effectiveness as a regularizer in many learning tasks, where the correlation among multiple latent embeddings requires to be jointly minimized or maximized. However, calculating precise TC values is challenging, especially when the closed-form distributions of embedding variables are unknown. In this paper, we introduce a unified framework to estimate total correlation values with sample-based mutual information (MI) estimators. More specifically, we discover a relation between TC and MI and propose two types of calculation paths (tree-like and line-like) to decompose TC into MI terms. With each MI term being bounded, the TC values can be successfully estimated. Further, we provide theoretical analyses concerning the statistical consistency of the proposed TC estimators. Experiments are presented on both synthetic and real-world scenarios, where our estimators demonstrate effectiveness in all TC estimation, minimization, and maximization tasks. The code is available at https://github.com/Linear95/TC-estimation.

==> figs/demo/draw.tex <==
\begin{table}
% \centering
% \begin{adjustbox}{width=0.45\columnwidth,center}
% \caption{Performance of mutual information estimation approaches on Gaussian.}
% \centering
% \begin{figure}
% \begin{figure}
% \end{wraptable}
% \begin{wrapfigure}{r}{0.45\textwidth}
   \begin{minipage}{.45\linewidth}
  \begin{subfigure}{.45\textwidth}
\includegraphics[width=\textwidth]{figs/demo/a1.pdf}
% \hspace{5pt}
\caption{MI-fix}
\end{subfigure}
  \begin{subfigure}{.45\textwidth}
\includegraphics[width=\textwidth]{figs/demo/a2.pdf}
\caption{MI-sample}
\end{subfigure}
% \end{minipage}
% \begin{minipage}{.5\linewidth}
  \begin{subfigure}{.3\textwidth}
\includegraphics[width=0.9\textwidth]{figs/demo/a3.pdf}
\caption{Core View}
\end{subfigure}
  \begin{subfigure}{.3\textwidth}
\includegraphics[width=0.9\textwidth]{figs/demo/a4.pdf}
\caption{Full Graph}
\end{subfigure}
  \begin{subfigure}{.3\textwidth}
\includegraphics[width=\textwidth]{figs/demo/a5.pdf}
  \caption{TC}
\end{subfigure}
% \caption{This is a image}
\captionof{figure}{Graphical models corresponding to methods of input augmentation combinations. \(A_1, A_2,A_3,A_4\) mean four input augmentations.
% \rhg{unclear sentence.}
Solid lines indicate the bivariate score function between connected nodes are considered during training. The number of solid lines represents the number of objectives.
% Dashed lines in (b) represents the corresponding node could be sampled. 
}
\label{fig:aug-structure}
\end{minipage}
\hspace{10pt}
\begin{minipage}{.45\linewidth}
% \begin{table}
% \centering
% \vspace{-5pt}
% \begin{adjustbox}{width=0.45\columnwidth}
% \begin{adjustbox}{width=\columnwidth,center}
\begin{tabular}{@{}lll@{}}
\toprule
\diagbox{Method}{Model} & BERT             & RoBERTa          \\ \midrule
MI-fix                                & 78.54$_{\pm 0.15}$   & 79.28$_{\pm 0.23}$ \\
MI-sample                               & 78.41$_{\pm 0.13}$  & 79.27$_{\pm 0.34}$ \\
Core View~\citep{tian2020contrastive}                                  & 78.64$_{\pm 0.22}$   & 79.41$_{\pm 0.25}$ \\
% Full Graph                                 & 78.52$_{\pm 0.13}$  & 79.68$_{\pm 0.20}$ \\
Full Graph~\citep{tian2020contrastive}                                & 78.52$_{\pm 0.13}$  &  79.49$_{\pm 0.26}$ \\
% Full Graph (sample)                        
TC                 & 78.72$_{\pm 0.10}$  & 79.58$_{\pm 0.25}$ \\ \bottomrule
\end{tabular}
% \end{adjustbox}
% \end{adjustbox}
% \end{table}
\vspace{6pt}
\caption{Ablation study on different information aggregation methods of augmentations.
Average Spearman's correlation score over 7 STS tasks is reported. MI is the abbreviation for mutual information. TC is the abbreviation for total correlation.\becky{align}}
% \vspace{5pt}
% \end{table}
\label{table:ablation}
\end{minipage}
\end{table}
% \end{wrapfigure}
% \end{figure}
% \end{minipage}
% \end{adjustbox}


==> figures/disen_pipeline.tex <==
\begin{wrapfigure}{l}{0.4\textwidth}
%   \begin{minipage}{.6\linewidth}
%   \begin{subfigure}{\textwidth}
\includegraphics[width=0.4\textwidth]{figs/disentangle_pipeline.pdf}
\caption{Pipeline of feature disentangle framework with $\TC$. $\vx$ is the input image, $\vz_c$, $\vz_d$< $\vz_s$ are latent representations which we want them to be disentangled. $\vx^\dag$ is the shuffled latent space and its decode image $\vx^\dag$ is treated as synthesized data for adversarial training.   }
\label{fig:disentangle_tc_pipeline}
\end{wrapfigure}


==> figures/disen_whole.tex <==
\begin{figure}[t]
\begin{minipage}{.5\textwidth}
    % \centering
\includegraphics[width=0.4\textwidth]{figs/disentangle_pipeline.pdf}
\caption{Pipeline of feature disentangle framework with $\TC$. $\vx$ is the input image, $\vz_c$, $\vz_d$< $\vz_s$ are latent representations which we want them to be disentangled. $\vx^\dag$ is the shuffled latent space and its decode image $\vx^\dag$ is treated as synthesized data for adversarial training.   }
    \label{fig:line-like-mse}
\end{minipage}
% \end{figure}
% \begin{figure}[t]
\begin{minipage}{.5\textwidth}
    % \centering
    \includegraphics[width=\textwidth]{figs/bias_variance_4d.pdf}
    \caption{Bias, variance and MSE of \textbf{tree-like} TC estimators.}
    \label{fig:tree-like-mse}
\end{minipage}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
